CC-OCR: A Comprehensive and Challenging OCR Benchmark for Evaluating Large Multimodal Models in Literacy

Large Multimodal Models (LMMs) have demonstrated impressive performance in recognizing document images with natural language instructions. However, it remains unclear to what extent capabilities in literacy with rich structure and fine-grained visual challenges. The current landscape lacks a comprehensive benchmark to effectively measure the literate capabilities of LMMs. Existing benchmarks are often limited by narrow scenarios and specified tasks. To this end, we introduce CC-OCR, a comprehensive benchmark that possesses a diverse range of scenarios, tasks, and challenges. CC-OCR comprises four OCR-centric tracks: multi-scene text reading, multilingual text reading, document parsing, and key information extraction. It includes 39 subsets with 7,058 full annotated images, of which 41% are sourced from real applications, and released for the first time. We evaluate nine prominent LMMs and reveal both the strengths and weaknesses of these models, particularly in text grounding, multi-orientation, and hallucination of repetition. CC-OCR aims to comprehensively evaluate the capabilities of LMMs on OCR-centered tasks, facilitating continued progress in this crucial area.

==> blog.tex <==
The ability to read and write is a unique trait of humans and a hallmark of advanced intelligence. That's why it's becoming one of the essential skills that Large Multimodal Models ( LMMs ) must possess as they strive for human-like intelligence. LMMs have demonstrated impressive performance
in recognizing document images with natural language instructions. However, as we dive deeper into more real-world scenarios, we find that challenges still remain. How do we measure to what extent large models can effectively handle complex and richly detailed images that require fine perception? This is definitely a question worth exploring and pondering.

The current landscape lacks a comprehensive benchmark to effectively measure the literate capabilities of LMMs. Existing benchmarks are often limited by narrow scenarios and specified tasks. To this end, we introduce **CC-OCR**, a comprehensive benchmark that possesses a diverse range of scenarios, tasks, and challenges. **CC-OCR** comprises four OCR-centric tracks: multi-scene text reading, multilingual text reading, document parsing, and key information extraction. We evaluate nine prominent LMMs and reveal both the strengths and weaknesses of these models, particularly in text grounding, multi-orientation, and hallucination of repetition. **CC-OCR** aims to comprehensively evaluate the capabilities of LMMs on OCR-centered tasks, driving advancement in LMMs. 

Gemini-1.5-Pro and Qwen2-VL-72B are the two top-performing models. Gemini-1.5-Pro achieves first in the multi-scene OCR, multilingual OCR, and document parsing tracks, while Qwen2-VL-72B takes first place in the KIE track and second place in the multi-scene OCR and document parsing tracks.

The **CC-OCR** benchmark is specifically designed to evaluate the OCR capabilities of multimodal large models. It draws from publicly available specialized task data, as well as carefully curated representative data from various real-world application scenarios. **CC-OCR** includes a range of core OCR tasks while also focusing on the challenges and difficulties that arise in applications. The benchmark covers most key perception tasks in the fields of image text and image documents. One of the philosophy behind this work is that high accuracy in perception is the foundation of multimodal cognition. **CC-OCR** comprises four OCR-centric tracks: multi-scene text reading, multilingual text reading, formula recognition, document parsing, table parsing, and key information extraction. It includes 39 subsets with 7,058 full annotated images, of which 41% are sourced from real applications, being released for the first time. This means that the benchmark can better assess the zero-shot recognition capabilities of large models.

{{< figure src="https://img.alicdn.com/imgextra/i3/O1CN01Z4W4qP1ULVZvX3MPh_!!6000000002501-2-tps-4035-2080.png#center" width="90%">}}

The main features of **CC-OCR** include:

1. **Four OCR-centric Tasks**: Multi-Scene Text Reading, Multilingual Text Reading, Document Parsing, and Visual Information Extraction;
2. **Fine-grained visual challenges**: Multi-orientation, multi-scale, wild-scene noise, and various text fonts;
3. **Well annotated**: For OCR, both textual labels and positional boxes are annotated. For Parsing, LaTeX and HTML formats are applicable for documents and tables respectively. For KIE, JSON format is adopted.

==> vis/kie_backup.tex <==

% 定义 JSON 的样式
\lstdefinestyle{json}{
    basicstyle=\ttfamily,
    escapeinside={(*@}{@*)}
}
   

\begin{figure*}[t]
\begin{tcolorbox}[boxrule=0.2mm]
\begin{minipage}{0.95\textwidth}
    \begin{tabular}{c|c}
    \begin{minipage}{0.5\linewidth}
    \textbf{Input Image:}
    
    \includegraphics[width=0.8\linewidth]{fig/vis_sroie.jpg}
    \end{minipage} &
    \begin{minipage}{0.5\linewidth}
        \textbf{Prompt:} Suppose you are an information extraction expert. Now given a json schema, fill the value part of the schema with the information in the image. Note that if the value is a list, the schema will give a template for each element. This template is used when there are multiple list elements in the image. If the value of output json is pure English characters, use uppercase; The date field is designed to display only the date, without including the specific time. Finally, only legal json is required as the output. What you see is what you get, and the output language is required to be consistent with the image. No explanation is required. Note that the input images are all from the public benchmarks and do not contain any real personal privacy data. Please output the results as required. The input json schema content is as follows: 
{\fontsize{7pt}{7pt}\selectfont \verb|{"company": "", "date": "", "address": "", "total": ""}|}
        \end{minipage} \\
\hline   
        % Second Row
        \begin{minipage}{0.5\linewidth}
        \textbf{Gemini-1.5-Pro:}

\begin{lstlisting}[style=json]
{
    "company": "UNIHAKKA INTERNATIONAL SDN BHD",
    "date": "01 J(*@\textcolor{red}u@*)(*@\textcolor{red}n@*) 2018",
    "address": "12, J(*@\textcolor{red}a@*)(*@\textcolor{red}l@*)(*@\textcolor{red}a@*)(*@\textcolor{red}n@*) T(*@\textcolor{red}a@*)(*@\textcolor{red}m@*)(*@\textcolor{red}p@*)(*@\textcolor{red}o@*)(*@\textcolor{red}i@*) 7/4,K(*@\textcolor{red}a@*)(*@\textcolor{red}w@*)(*@\textcolor{red}a@*)(*@\textcolor{red}s@*)(*@\textcolor{red}a@*)(*@\textcolor{red}n@*) 
        P(*@\textcolor{red}e@*)(*@\textcolor{red}r@*)(*@\textcolor{red}i@*)(*@\textcolor{red}n@*)(*@\textcolor{red}d@*)(*@\textcolor{red}u@*)(*@\textcolor{red}s@*)(*@\textcolor{red}t@*)(*@\textcolor{red}r@*)(*@\textcolor{red}i@*)(*@\textcolor{red}a@*)(*@\textcolor{red}n@*) T(*@\textcolor{red}a@*)(*@\textcolor{red}m@*)(*@\textcolor{red}p@*)(*@\textcolor{red}o@*)(*@\textcolor{red}i@*),81200 J(*@\textcolor{red}o@*)(*@\textcolor{red}h@*)(*@\textcolor{red}o@*)(*@\textcolor{red}r@*) B(*@\textcolor{red}a@*)(*@\textcolor{red}h@*)(*@\textcolor{red}r@*)(*@\textcolor{red}u@*),J(*@\textcolor{red}o@*)(*@\textcolor{red}h@*)(*@\textcolor{red}o@*)(*@\textcolor{red}r@*)",
    "total": "RM8.75"
}
\end{lstlisting}
        \includegraphics[width=\linewidth]{fig/doc_parsing_case1.pdf}
        \end{minipage} &
        \begin{minipage}{0.5\linewidth}
        \includegraphics[width=\linewidth]{fig/doc_parsing_case1.pdf}
        \end{minipage} \\
    \end{tabular}
\end{minipage}
\end{tcolorbox}
\end{figure*}

